MLP Architectures for Vision-and-Language Modeling: An Empirical Study

We initiate the first empirical study on the use of MLP architectures for vision-and-language (VL) fusion. Through extensive experiments on 5 VL tasks and 5 robust VQA benchmarks, we find that: (i) Without pre-training, using MLPs for multimodal fusion has a noticeable performance gap compared to transformers; (ii) However, VL pre-training can help close the performance gap; (iii) Instead of heavy multi-head attention, adding tiny one-head attention to MLPs is sufficient to achieve comparable performance to transformers. Moreover, we also find that the performance gap between MLPs and transformers is not widened when being evaluated on the harder robust VQA benchmarks, suggesting using MLPs for VL fusion can generalize roughly to a similar degree as using transformers. These results hint that MLPs can effectively learn to align vision and text features extracted from lower-level encoders without heavy reliance on self-attention. Based on this, we ask an even bolder question: can we have an all-MLP architecture for VL modeling, where both VL fusion and the vision encoder are replaced with MLPs? Our result shows that an all-MLP VL model is sub-optimal compared to state-of-the-art full-featured VL models when both of them get pre-trained. However, pre-training an all-MLP can surprisingly achieve a better average score than full-featured transformer models without pre-training. This indicates the potential of large-scale pre-training of MLP-like architectures for VL modeling and inspires the future research direction on simplifying well-established VL modeling with less inductive design bias. Our code is publicly available at: https://github.com/easonnie/mlp-vil

==> tables/archive/main_table.tex <==

\begin{table*}[t]
    \centering
    \small\resizebox{\textwidth}{!}{
    \begin{tabular}{lcclccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}}
    % & \multirow{2}{*}{\textbf{Visual Encoder}}
    % & \multirow{2}{*}{\textbf{Text Encoder}}
    % & \multirow{2}{*}{\textbf{Fusion}}
    & \multicolumn{3}{c}{\textbf{Flickr30K (IR)}} & \multicolumn{3}{c}{\textbf{Flickr30K (TR)}}% 6-12, 7-13
    & \multicolumn{2}{c}{\textbf{VQA}}
    & \multicolumn{2}{c}{\textbf{GQA}}
    & \multicolumn{2}{c}{\textbf{SNLI-VE}}
    & \multicolumn{2}{c}{\textbf{NLVR$^2$}}\\
    
    % & \multicolumn{3}{c}{B} 
    % & \multicolumn{3}{c}{C}\\
    % \cmidrule(rl){7-12}
    %  & & & & & \multicolumn{3}{c}{\textbf{IR}} & \multicolumn{3}{c}{\textbf{TR}} \\
    % \cmidrule(rl){5-7}\cmidrule(rl){8-10}
    % \cmidrule(rl){7-9}\cmidrule(rl){10-12}
      & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & test-dev & test-std & test-dev & test-td  & dev & test & dev & test-p\\
    % & \textbf{JSD$\downarrow$} & \textbf{KL$\downarrow$} & \textbf{Acc.$\uparrow$ } & \textbf{JSD$\downarrow$} & \textbf{KL$\downarrow$} & \textbf{Acc.$\uparrow$ } & \textbf{JSD$\downarrow$} & \textbf{KL$\downarrow$} & \textbf{Acc.$\uparrow$ }\\
    % \midrule
    % wo pretrain & ResNet50$\times$4 (CLIP) & RoBERTa-base & Transformers & 74.04 \\
    % w pretrain & ResNet50$\times$4 (CLIP) & RoBERTa-base & Transformers & 75.30 (+1.26) \\
    % wo pretrain & ResNet50$\times$4 (CLIP) & RoBERTa-base & MLPs & 67.47 \\
    % w pretrain & ResNet50$\times$4 (CLIP) & RoBERTa-base & MLPs & 73.20 (+5.73) \\
    % wo pretrain & ResNet50$\times$4 (CLIP) & RoBERTa-base & MLPs + tiny att. & 73.80 \\
    % w pretrain & ResNet50$\times$4 (CLIP) & RoBERTa-base & MLPs + tiny att. & 74.77 (+0.97)\\
    % \midrule
    % wo pretrain & SwinMLP & Embeddings & MLPs &  \\
    % w pretrain & SwinMLP & Embeddings & MLPs & \\
    % \midrule
    \hline
    \hline
    \multicolumn{12}{l}{\textit{Previous models with pre-training}}\\
    \hline
    UNITER &  72.5 &  92.4 & 96.1 &85.9 & 97.1 & 98.8 & 72.70 & 72.91  & 59.99 & - & 78.59 &  78.28 & 77.18 & 77.85\\
    VinVL & - & - & -& - & - & - & 75.95 & 76.12 & \textbf{65.05} & \textbf{65.65}  & - & -  & 82.05 & 83.08\\
    ViLT & 64.4 & 88.7 & 93.8 &  83.5 & 96.7 & 98.6 & 71.26 & - & - & -  & - & -  &  75.70  & 76.13\\
    CLIP-ViL & - & - & - & - & - & - &  \textbf{76.48} & \textbf{76.70} & 61.42  & 62.93 & \textbf{80.61} & \textbf{80.20}  & - & -\\
    % \midrule
    \hline
    \hline
    \multicolumn{12}{l}{\textit{Our models (different architectures for vision and language fusion) w/o pre-training}}\\
    \hline
    Transformer & - & - & - & - & - & - &  74.04&  & 58.58 & & 78.44 & 78.69 & 54.03 & 52.30\\
    MLP & - & - & - & - & - & - &  67.47 &  & 54.14 & & 77.24 & 76.98 & 54.41 & 52.51\\
    MLP + tiny att. & - & - & - & - & - & - &  73.80 &  & 59.35 & & 78.32 & 78.30 & 53.90 & 51.90\\
    % \midrule
    \hline
    \hline
    \multicolumn{12}{l}{\textit{Our models (different architectures for vision and language fusion) with pre-training}}\\
    \hline
    Transformer & 73.78 & 93.52 & 96.46 & 89.00 & 98.20 & 99.40 & 75.42 (+1.38)& 75.74 & 61.33 & & 79.64 & 79.90 & 79.55 & 78.36\\
    MLP & 65.42 & 91.20 & 95.26 & 78.90 & 97.50 & 99.20 &  73.20 (+5.73)  & 73.44 & 58.30 & & 78.48 & 78.01 & 73.22 & 74.32\\
    MLP + tiny att. & 73.78 & 93.76 & 97.06 & 88.11 & 98.40 & 99.50 & 74.77 (+0.97)& 74.93 & 61.28  & & 79.50 &  79.32 & 76.23 & 77.92\\
    \hline
    \hline
    \multicolumn{12}{l}{\textit{Full MLP with pre-training (Permutator MLP)}}\\
    \hline
    Full MLP & 42.68 & 75.08 & 83.82 & 55.74 & 85.61 & 91.91 & ~64.28\yixin{update later} & & 52.53 & & 74.07 & 74.05 & 66.92 & 66.94\\
    Full MLP + tiny att. & 57.40 & 85.40 & 91.00 & 72.62 & 92.16 & 95.93 & ~67.27\yixin{update later}& & 55.83 & & 75.03 & 75.13 & 72.72 & 71.36 \\
    \hline
    \hline
    \multicolumn{13}{l}{\textit{Full MLP with pre-training (Swin MLP) }}\\
    \hline
    Full MLP & 50.52  & 79.96 & 88.16 & 66.23 & 89.01 & 93.41 & ~65.36\yixin{update later} & & 54.45  & & 75.21 & 75.02 & 68.82 & 67.96\\
    Full MLP + tiny att. & 59.50 & 85.88 & 92.08 & 76.62 & 93.11 & 96.50 & ~68.96\yixin{update later} & & 57.35 & & 75.92  & 75.39 & 73.37 & 72.70 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Main Results (The key findings in the main table is that (1). There are noticeable performance gap between Transformer and MLP if we do not pretrain the models. However, such performance gap can be closed by adding very light-weighted tiny att.; (2). After pretraining, MLP is able to get very close performance as transformers.; (3) Models with MLP fusion can give similar performance as previous state-of-the-art.) \linjie{Full MLP running}}
    \label{tab:main}
\end{table*}
